High-quality Task Division for Large-scale Entity Alignment

Entity Alignment (EA) aims to match equivalent entities that refer to the same real-world objects and is a key step for Knowledge Graph (KG) fusion. Most neural EA models cannot be applied to large-scale real-life KGs due to their excessive consumption of GPU memory and time. One promising solution is to divide a large EA task into several subtasks such that each subtask only needs to match two small subgraphs of the original KGs. However, it is challenging to divide the EA task without losing effectiveness. Existing methods display low coverage of potential mappings, insufficient evidence in context graphs, and largely differing subtask sizes. In this work, we design the DivEA framework for large-scale EA with high-quality task division. To include in the EA subtasks a high proportion of the potential mappings originally present in the large EA task, we devise a counterpart discovery method that exploits the locality principle of the EA task and the power of trained EA models. Unique to our counterpart discovery method is the explicit modelling of the chance of a potential mapping. We also introduce an evidence passing mechanism to quantify the informativeness of context entities and find the most informative context graphs with flexible control of the subtask size. Extensive experiments show that DivEA achieves higher EA performance than alternative state-of-the-art solutions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/note.tex <==
\section{Note}

This is my note and will be deleted later.

\begin{table}
    \caption{Symbols}
    \begin{tabular}{|c|c|}
        \hline
        Symbol & Explaination \\
        \hline
        $\mathcal{G}=\langle E, R, T \rangle$ & KG consisting of Entity, Relation, Triple sets. \\
        $\mathcal{G}^s, \mathcal{G}^t$ & Source KG and target KG \\
        $\widetilde{\mathcal{G}}, \widetilde{E}$ & Subgraph and its Entity set \\
        $E^{u}, E^{a}$ & unmatched entities, anchor entities  \\
        $M^l, M^p$ & Labelled and predicted mappings \\
        $s,t,l,p,'$ & superscripts (consider using mathrm) \\
        $S$ & Size limitation of each subtask \\
        $|E|$ & Entity number \\
        $m,h$ & message passing \\
        $\alpha, \beta, \lambda_1, \lambda_2$ & hyperparameters \\
        $\theta$ & parameters \\
        $W$ & entity weight \\
        \hline
    \end{tabular}
\end{table}



\begin{table}
    \caption{Terms}
    \begin{tabular}{|c|c|}
        \hline
        Terms & Writing \\
        \hline
        Knowledge Graph &  \\
        Entity Alignment &  \\
        Division of EA & \\
        Source KG, target KG & \\
        Task, subtask & \\
        Counterpart candidates & \\
        Evidence & \\
        Anchor, linking entities & \\
        Select counterpart candidates & \\
        Build context & \\
        Locality & \\
        Graph, subgraph, context graph & \\
        Mappings & \\
        Source anchor, target anchor & \\
        coherence & \\
        \hline
    \end{tabular}
\end{table}








==> sections/tables/compare_ctx.tex <==
\scalebox{1}[1]{
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{DBP15K(FR-EN)} & \multicolumn{3}{c|}{DBP15K(JA-EN)} & \multicolumn{3}{c|}{DBP15K(ZH-EN)} & \multicolumn{3}{c|}{DWY100K(DBP-WD)} & \multicolumn{3}{c}{DWY100K(DBP-YG)}  \\
        & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR\\
        \hline
        Graph Partition & & & & & & & & & & & & & & & \\
        \hline
        Ours & & & & & & & & & & & & & & & \\
        \hline
    \end{tabular}
    }

==> sections/tables/couterdiscovery_ablation.tex <==
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Method} &\multicolumn{2}{c|}{FR-EN}&\multicolumn{2}{c|}{JA-EN}&\multicolumn{2}{c|}{ZH-EN}&\multicolumn{2}{c|}{DBP-WD}&\multicolumn{2}{c}{DBP-YG} \\
    & Recall & MRR& Recall & MRR& Recall & MRR& Recall & MRR& Recall & MRR \\
    \hline
    Locality & 0.737&0.591&0.752&0.589&0.722&0.577&0.677&0.53&0.735&0.637 \\
    Similarity &0.561&0.515&0.555&0.506&0.555&0.511&0.564&0.514&0.696&0.663 \\
    Locality+Similarity &0.882&0.709&0.89&0.703&0.884&0.706&0.825&0.663&0.886&0.775 \\
    \hline
\end{tabular}



==> sections/tables/mem_n_time.tex <==
\begin{tabular}{c|ccccc|ccccc}
    \hline
    \multirow{2}{*}{EA model} & \multicolumn{5}{c|}{Time} & \multicolumn{5}{c}{GPU memory} \\
    & 1 & 2 & 3 & 4 & 5 & 1 & 2 & 3 & 4 & 5 \\
    \hline
    GCN-Align & & & & & & & & & & \\
    RREA & & & & & & & & & &  \\
    \hline
\end{tabular}





==> sections/tables/over_perf_dbp.tex <==
\scalebox{1}[1]{
    \begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc}
        \hline
        \multirow{2}{*}{EA model} &\multirow{2}{*}{Method} & \multicolumn{3}{c|}{DBP15K(FR-EN)} & \multicolumn{3}{c|}{DBP15K(JA-EN)} & \multicolumn{3}{c|}{DBP15K(ZH-EN)} & \multicolumn{3}{c|}{DWY100K(DBP-WD)} & \multicolumn{3}{c}{DWY100K(DBP-YG)}  \\
        & & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR & H@1 & H@5 & MRR\\
        \hline
        \multirow{5}{*}{GCN-Align} & LargeEA & 0.282&0.485&0.374&0.205&0.35&0.271&0.307&0.493&0.393&0.17&0.272&0.215&0.14&0.206&0.17 \\
        & LargeEA (semi) & 0.355&0.538&0.439&0.258&0.388&0.318&0.37&0.533&0.446&0.29&0.415&0.346&0.226&0.304&0.262 \\
        & LIME & & & & & & & & & & & & & & & \\
        & LIME (semi) & & & & & & & & & & & & & & & \\
        \hline
        & Ours & 0.396&0.644&0.505&0.405&0.646&0.511&0.374&0.606&0.476&0.393&0.568&0.472&0.549&0.694&0.615 \\
        \hline
        \hline
        \multirow{5}{*}{RREA} & LargeEA & 0.501&0.67&0.576&0.414&0.553&0.477&0.515&0.667&0.583 &0.381&0.467&0.42&0.356&0.432&0.39  \\
        & LargeEA (semi) & 0.565&0.704&0.628&0.447&0.562&0.5&0.568&0.698&0.628 &0.413&0.486&0.446&0.38&0.446&0.409 \\
        & LIME & & & & & & & & & & & & & & & \\
        & LIME (semi) & & & & & & & & & & & & & & & \\
        \hline
        & Ours & 0.644&0.795&0.71&0.633&0.789&0.701&0.632&0.78&0.697&0.615&0.724&0.664&0.745&0.832&0.785 \\
        \hline
    \end{tabular}
    }

==> sections/tables/over_perf_ids.tex <==
\scalebox{0.85}[0.85]{
    \begin{tabular}{c|ccccc|ccccc|ccccc|ccccc}
        \hline
        \multirow{2}{*}{Method} & \multicolumn{5}{c|}{IDS15K(EN-FR)} & \multicolumn{5}{c|}{IDS15K(EN-DE)} & \multicolumn{5}{c|}{IDS100K(EN-FR)} & \multicolumn{5}{c}{IDS100K(EN-DE)}  \\
        & H@1 & H@5 & MRR & Time & Mem. & H@1 & H@5 & MRR & Time & Mem. & H@1 & H@5 & MRR & Time & Mem. & H@1 & H@5 & MRR & Time & Mem. \\
        \hline
    \end{tabular}
    }
